On Some Generalized Vertex Folkman Numbers

For a graph $G$ and integers $a_i\ge 1$, the expression $G \rightarrow (a_1,\dots,a_r)^v$ means that for any $r$-coloring of the vertices of $G$ there exists a monochromatic $a_i$-clique in $G$ for some color $i \in \{1,\cdots,r\}$. The vertex Folkman numbers are defined as $F_v(a_1,\dots,a_r;H) = \min\{|V(G)| : G$ is $H$-free and $G \rightarrow (a_1,\dots,a_r)^v\}$, where $H$ is a graph. Such vertex Folkman numbers have been extensively studied for $H=K_s$ with $s>\max\{a_i\}_{1\le i \le r}$. If $a_i=a$ for all $i$, then we use notation $F_v(a^r;H)=F_v(a_1,\dots,a_r;H)$. Let $J_k$ be the complete graph $K_k$ missing one edge, i.e. $J_k=K_k-e$. In this work we focus on vertex Folkman numbers with $H=J_k$, in particular for $k=4$ and $a_i\le 3$. A result by Ne\v{s}et\v{r}il and R\"{o}dl from 1976 implies that $F_v(3^r;J_4)$ is well defined for any $r\ge 2$. We present a new and more direct proof of this fact. The simplest but already intriguing case is that of $F_v(3,3;J_4)$, for which we establish the upper bound of 135 by using the $J_4$-free process. We obtain the exact values and bounds for a few other small cases of $F_v(a_1,\dots,a_r;J_4)$ when $a_i \le 3$ for all $1 \le i \le r$, including $F_v(2,3;J_4)=14$, $F_v(2^4;J_4)=15$, and $22 \le F_v(2^5;J_4) \le 25$. Note that $F_v(2^r;J_4)$ is the smallest number of vertices in any $J_4$-free graph with chromatic number $r+1$. Most of the results were obtained with the help of computations, but some of the upper bound graphs we found are interesting by themselves.

==> exi.tex <==
\section{The Existence of $F_v(3^r;J_4)$ and $F_e(3,3;H)$}

Two seminal papers by Ne\v{s}et\v{r}il and R\"{o}dl~\cite{NR76,NR81}
lay the foundation for our reasoning
in this section: the first one from 1976 implies that
the edge Folkman numbers $F_e(3^r;K_4)$ are well defined
for all $r \ge 1$, and the second paper from 1981 shows
that $F_v(3,3;J_4)$ is well defined. These, together with
a technique developed by Dudek and R\"{o}dl in 2008~\cite{DR08},
permit us to give a rather elementary proof that
$F_v(3^r;J_4)$ is well defined for all $r \ge 1$.

For graph $G = (V_G,E_G)$, we define the graph $F=DR(G)$
as in the construction by Dudek-R\"{o}dl \cite{DR08}, as follows:
$$DR(G) = F = (E_G,E_F),$$
where the set of vertices of $F$ consists of
the edges of $G$, and the edge set $E_F$ contains
the edges $\{ef, fg, eg\}$
for every edge-triangle $efg$ in $E_G$, and no other edges.
Note that each pair of edges from triangle
$\{e, f, g\} \subseteq E_G$
spans the same three vertices in $G$,
and thus the same three vertices in
the corresponding vertex-triangle in $F$.
Such triangles in $F$ will be called {\em images}
of triangles from $G$,
other triangles in $F$ will be called {\em spurious}.
Note that for any edge $ef$ in $E_F$, the edges $e$ and $f$ in $E_G$
must share one vertex.
It is easy to observe (see the proof of Lemma~\ref{l:DRG}(2) below)
that two image triangles may share vertices but
no edges.

\smallskip
\noindent
\emph{Example.}
For $G=K_4$, $DR(G)$ has 6 vertices, 12 edges
(it is 4-regular), and 8 triangles. These 8 triangles
are split into 4 images of triangles from $G$
and 4 spurious triangles.

\begin{lemma}
\label{l:DRG}
Let $G$ be any $K_4$-free graph, and let $F$ denote
the graph $DR(G)$. Then we have that:

\begin{enumerate}
    \item $F$ has no spurious triangles,
    \item $F$ is $J_4$-free, and
    \item $G \rightarrow (3^r)^e$ if and only if $F \rightarrow (3^r)^v$,
for every $r \ge 1$.
\end{enumerate}
\end{lemma}

\begin{proof}
First, we will show that the graph $F=DR(G)$
has no spurious triangles.
For contradiction, suppose that $efg$ is a spurious triangle in $F$,
where $e=\{A,B\}$ and $f=\{A,C\}$ for some vertices $A,B,C \in V_G$.
Since edge $g$ is incident to both $e$ and $f$, but $efg$ is not
an image of a triangle in $G$, we must have $g=\{A,D\}$ for
another vertex $D \in V_G$. This implies that $ABC, ABD, ACD$ are
triangles, and thus also $BCD$, in $G$. Hence $ABCD$ forms a $K_4$
in $G$, contradicting the assumption. This shows part (1).

If $F$ contains $J_4$ with the vertices $\{e,f,g,h\}$ and
formed by two triangles $\{efg\}$ and $\{efh\}$, then we
claim that at most one of them is an image triangle.
In order to see this, let $e=\{A,B\}$, $f=\{A,C\}$ and note
that the unique image triangle in $F$ containing $e$ and $f$
is the one implied by the triangle $ABC$ in $G$.
Hence, at least one of $\{efg\}$ and $\{efh\}$ must
be spurious, but by (1) this is impossible in $F=DR(G)$
obtained from a $K_4$-free graph $G$. Thus (2) follows.

For (3),
consider the natural bijection between all
$r$-vertex-colorings of $F$ and $r$-edge-colorings
of $G$. This bijection
preserves the number of colors used in any edge-triangle
in $G$ when mapped to its image triangle
in $F$. Hence, because of (1) and (2), we can conclude (3).
\end{proof}

Using Lemma \ref{l:DRG}, we can give a simple proof
that for every $r$ there exists a $J_4$-free graph
such that in any $r$-coloring of its vertices
there must be a monochromatic triangle, or
equivalently, $\mathcal{F}_v(3^r;J_4) \not=\emptyset$.


\noindent
{\em Proof of Theorem~\ref{t:3rj4}}.
A general result by Ne\v{s}et\v{r}il and R\"{o}dl~\cite{NR76}
implies that the sets $\mathcal{F}_e(3^r;K_4)$ are
nonempty for all $r \ge 1$. This, together with the claim
that $\mathcal{F}_v(3^2;J_4) \not=\emptyset$, was also
discussed in~\cite{XLR18}. For general $r$, consider
any graph $G \in \mathcal{F}_e(3^r;K_4)$.
Then by Lemma~\ref{l:DRG}(3), we have that
$DR(G) \in \mathcal{F}_v(3^r;J_4)$,
and thus the numbers of the form
$F_v(3^r;J_4)$ are well defined for all $r \ge 1$.
\hfill$\square$


Note that, by monotonicity, Theorem~\ref{t:3rj4} implies
the existence of Folkman numbers of the form
$F_v(a_1,\dots,a_r;J_4)$ with
$1 \le a_i \le 3$ for all $1 \le i \le r$.
The orders of graphs in $\mathcal{F}_e(3^r;K_4)$
and $\mathcal{F}_v(3^r;J_4)$ can be expected to be quite
large, even for small $r$. In the trivial case for $r=1$
we have $F_e(3;K_4)=F_v(3;J_4)=3$, but both problems become
very difficult already for $r=2$. For the edge problem,
the best known bounds are $21 \le F_e(3,3;K_4) \le 786$~\cite{BN20,LRX14},
while for the vertex problem we establish
the bound $F_v(3,3;J_4) \le 135$ in Theorem~\ref{t:33j4}.
We are not aware of any reasonable bounds
for $r \ge 3$ in either case.


We wish to point to a study of the existence
of edge Folkman numbers for some small parameters \cite{XLR18}. While a simple argument
easily shows that $F_e(3,3;J_4)$ does not exist,
for other cases with $|V(H)|\le 5$ one can prove
or disprove the existence of $F_e(3,3;H)$
with some work, leaving only two open cases.
Namely, the following is known:
the sets $\mathcal{F}_e(3,3;H)$ are nonempty for
all connected graphs $H$ containing $K_4$, and for
some graphs not containing $K_4$.
If $H$ is any connected $K_4$-free graph on
$5$-vertices containing $K_3$,
then $\mathcal{F}_e(3,3;H)=\emptyset$
except for two possible cases:
the wheel graph $W_5=K_1+C_4$ and its subgraph
$\overline{P_2 \cup P_3} \subset W_5$.
The latter two cases remain open.

==> spr.tex <==
\section{The existence of $F_v(K_3,\cdots,K_3;J_4)$}

\begin{verbatim}

On Sunday, 18 August 2019 22:58:30 EDT xxdmaths@sina.com wrote:
> 1. There is not interesting known upper bounds for the following Folkman
> numbers. It is interesting to know which among them are feasible to
> compute? a. F_e(3,4;5);b. F_v(K4,K4;K5-e);c. F_e(K4,K4;K5-e);
> Maybe b is easier than the other two. More results will make the paper
> better :-)

> 2. Have you found new upper bound for F_v(K3,K3;K4-e) better than 136?

Yes, I am attaching a good graph on 135 vertices. I have searched thousands of
graphs on 134 vertices and have not found anything so it looks like the random
approach will not help much more.

> The lower bound seems difficult, and the known lower bound is only 25.

> We can generate a $K_4-e$-free subgraph H of G_127, the known K_4-free graph with
> independence number 11, by a way similar to the $K_4-e$-free process, then generate
> a $K_4-e$-free graph G of order 134 by adding 7 vertices and more edges.
> If one of them arrows (3,3)^v, then we can generate smaller graphs similarly.

From:   	"David E. Narvaez" <den9562@rit.edu>
Date:   	Tue, August 27, 2019 12:57 pm

I checked all of the attached graphs and none of them arrow (3,3)^v.

----------------------------------------

Notation: Jk=Kk-e.

Problem 1. How to show that a J4-free graph arrows (3,3)^v?

The approach via SAT is effective, but it would be nice to
have some general properties. We may consider relationships
between n/e/t (number of vertices, edges and triangles) in
known cases. Any new nontrivial sufficient or necessary
constraints will be great.

Problem 2. Does there exist a J4-free graph G such that
every set of |V(G)|/2 induces a triangle? If not, this
could help analyzing F_v(K3,K3;J4).

F_e(K3,K3;J4) does not exist (simple argument).

We have a graph showing F_v(K3,K3;J4) <= 135
This easily implies F_v(K2,K2,K3;J4) <= 135

----------

JLX manuscript proves some implications between various
scenarios of arrowing. Together with computations they give:

F_v(K2,K3;J4) = 19

F_v(K2,K2,K2;J4) = 10
F_v(K2,K2,K3;J4) >= F_v(K3,K3;J4) >= 25

----------

Do we have anything on
F_v(K2,K3,K3;J4) or F_v(K3,K3,K3;J4)?

Suppose G -> (K3,K3)^v and G is J4-free. Take H to be
induced in G by non-neighbors of any vertex in G. Then
H -> (K2,K3)^v.

No upper bounds are known for the following
   a. F_e(K3,K4;K5)
   b. F_v(K4,K4;J5)
   c. F_e(K4,K4;J5)
Likely b is easier than the other two.

---------------------------------------------------

Subject:   	J5-free graphs
From:   	xxdmaths@sina.com
Date:   	Mon, September 2, 2019 9:51 pm

interesting upper bound for edge Folkman number
we discussed recently are more difficult than improving
the known upper bound on F_e(3,3;4).
For Fe(3,4;5), we may find a K_5-free graph in the survey on small Ramsey numbers
by Staszek. But the computation may be difficult.
Fv(K2,K2,K3;J4) may be much smaller than 135. But it is difficult to compute the
exact value because there are too many graph to deal with in computing the lower
bound.  So I suggest we work on Fv(K4,K4;J5), together the upper bound on
Fv(K3,K3;J4) obtained by David, and try to prove some related results (I am working
on it).
We may try other Folkman numbers considered recently, but
it is difficult to obtain an interesting upper bound or the exact value. Yu Jiang
sent me a few K_5-e-free graphs. The orders are 200, 230, 250, 270 and 300.
Please find the graphs in the attachment of this email, and test if they arrow
(4,4)^v.

--------------------------------------------

\end{verbatim}

A step forwards on a question we had a couple weeks ago,
the existence of $F_v(K_3,K_3,K_3;J_4)$. The proof is elementary
but can make a nice part of a paper.
For graph $G = (V_G,E_G)$, we define graph $DR(G)=H$ based on
a 2008 construction by Dudek-R\"{o}dl, as follows:

$$DR(G) = H = (E_G,E_H),$$

\noindent
where the set of vertices of $H$ consists of
the edges of $G$, and the set $E_H$ contains
the edges $\{ef, fg, eg\}$
for every edge-triangle $efg$ in G.
Note that each pair from such a
triangle in $H$, $\{e, f, g\} \subset E_G$,
spans the same three vertices in $G$.
Such triangles in $H$ are called images
of triangles from $G$,
other triangles in $H$ are called spurious.


\noindent
{\bf Example.}
For $G=K_4$, $DR(G)$ has 6 vertices, 12 edges
(it is 4-regular), and 8 triangles. These 8 triangles
are split into 4 images of triangles from $G$
and 4 spurious triangles.

\begin{lemma}
If graph $G$ is $K_4$-free, then $H=DR(G)$
is $J_4$-free, furthermore we have that:
$(1)$ all triangles in $G$ have images in $H$, so that
two images may share vertices but no edges.
$(2)$ $H$ as no spurious triangles.
\end{lemma}
\begin{proof}
Obvious by using some drawings on a napkin. Still,
a few smart lines will need to be written.
\end{proof}

\begin{theorem}
There exist graphs $H$ in $F_v(K_3,K_3,K_3;J_4)$.
\end{theorem}
\begin{proof}
It is known that $F_e(K_3,K_3,K_3;K_4)$ is nonempty.
We claim that for any graph $G$ in $F_e(K_3,K_3,K_3;K_4)$
we have $DR(G)$ in $F_v(K_3,K_3,K_3;J_4)$.

Let $H = DR(G)$. By Lemma we know that $H$ is $J_4$-free.
Note that the sets of 3-vertex-colorings of $H$ and
3-edge-colorings of $G$ are essentially the same.
We know that every 3-edge coloring of $G$ has a
monochromatic edge-triangle $efg$, thus its image
is also a monochromatic vertex-triangle in $H$.
\end{proof}

The above theorem easily generalizes to any number
of colors, i.e. for every $r$ there exists $J_4$-free
graphs whose any vertex coloring with $r$ color
contains monochromatic triangles. The orders of
such graphs can be expected to be very large.

\begin{verbatim}
I don't think Nesetril/Rodl would write about such concrete bounds.
This 157 may come from some reasoning of Xiaodong, or even it could be
from one of the cases Xiaodong asked you to solve. I do not have any emails
on this subject (including string 157), thus anything I wrote about it seemed
not important enough to save. Could I see a copy of this email?

January 30, 2020 3:35 PM, "David E. Narvaez" <den9562@rit.edu> wrote:

     I am working on including the work with Xiaodong as a subsection in my chapter 
     on arrowing but I have a question regarding an email of yours last year where 
     you ask if the current bound is Fv(3,3;J4) <= 157. Do you get that bound from the 
     construction of Ne and Rodl? (Theorem 3 in 
     https://arxiv.org/abs/1705.06268) Or is there some other work that covers that 
     case?
     
Can we get a bound on Fv(K4,K4;J5) using similar method?

Possibly, we could use a small case of Fv(K3,K3;J5) and describe
it in the paper (it is on at most 14 vertices).

Can we get any reasonable upper bound on F_v(K3,K3,K3;J4)?

---------------------

David E. Narvaez (April 8, 2020 7:54 PM)

I wanted to return to the work we did around June/July 2019 on Fv(K3,K3;J4). 

the part of the work I did with Fv(K3,K3;J4) 
is precisely the topic of my thesis I am very interested in including that 
result as part of the document. In order to properly do so, I believe we 
should at least publish a brief note with all the authors involved (including 
Yu Jiang). This note should be in some journal that accepts ancillary files, as 
we will need to provide the graph, the Boolean formula encoding the coloring 
property, and a proof of unsatisfiability.

\end{verbatim}


==> tail.tex <==
\section{Remarks and Some Open Problems}

Obtaining good bounds for concrete vertex Folkman numbers is
often difficult. The results presented in this paper are special
for the parameters involving $J_4$ but we hope that they may extend
to other or more general vertex cases. The techniques used here might
be not easily transferable to obtain new bounds on edge Folkman numbers,
not the least because just testing edge-arrowing is typically much more
difficult than testing vertex-arrowing.

\bigskip
We close this paper by posing some related open problems.

\begin{problem}\label{lower}
Give a general lower bound for $F_v(3^r;J_4)$,
or any nonobvious lower bound for $F_v(3,3;J_4)$,
which are not easily implied by known bounds for
other more studied parameters.
\end{problem}


Similarly, we do not know much about the cases
like $F_v(2^r;K_4)$, $F_v(3^r;K_4)$, or $F_v(4^r;J_5)$:
no general methods are known to obtain good lower
or upper bounds. 


\begin{problem}
Does there exist a $J_4$-free graph $G$ such that
every set of $|V_G|/2$ vertices induces a triangle? 
\end{problem}

\noindent
If not, this could help in the analysis of $F_v(3,3;J_4)$.
We may consider this problem in a more general case. 
By using density arguments, it is known how to obtain
upper bounds on $F_v(3^r;K_4)$, but not
on $F_v(3,3;J_4)$ or $F_v(3^r;J_4)$.

%Beyond $J_4$-free graphs: 
%
%$F_v(6,6;J_7) \le 5F_v(3,3;J_4)$, so now we have
%
%$F_v(6,6;J_7) \le 5*135=675$
%
%Is it feasible to improve 675 by computing?


Except for $F_e(3,4;K_5) \ge 22$ \cite{XS10},
we do not know of any other nonobvious bounds for:
(a) $F_v(3,4;J_5)$, (b) $F_v(4,4;J_5)$, 
(c) $F_e(3,4;K_5)$, or (d) $F_e(4,4;J_5)$.
Case (a) might be solvable with computational methods.
We also think that case (b), while far from easy, is easier
than (c) and much easier than (d). For a
similar case of $F_v(4,4;K_5)$,
the best known bounds were obtained in \cite{Bik18,Fv445}:
$$19 \le F_v(2,2,2,4;K_5) \le F_v(4,4;K_5) \le 23.$$


Finally, we state a related existence problem, which
was already raised in an earlier work \cite{XLR18},
and which is also described at the end of Section 2.

\begin{problem}
{\rm (a)}
$\mathcal{F}_e(3,3;K_1+C_4)=\emptyset?$
\hspace{.3cm}
{\rm (b)}
$\mathcal{F}_e(3,3;\overline{P_2 \cup P_3})=\emptyset?$
\end{problem}
We note that the YES answer to part (a) implies YES answer
to part (b), which eliminates one YES/NO combination
of answers (out
of four possible ones). This problem can be rephrased in
some interesting ways. For example,
part (a) is equivalent to the following question:
{\em Does there exist any $W_5$-free graph
which is not a union of two triangle-free graphs?}

\section*{Acknowledgement}

This research was partially supported by
the National Natural Science Foundation of China (11361008).
David E. Narváez was supported by NSF grant CCF-2030859 to the
Computing Research Association for the CIFellows Project.
